A Multi-Language Perspective on the Robustness of LLM Code Generation

Large language models have gained significant traction and popularity in recent times, extending their usage to code-generation tasks. While this field has garnered considerable attention, the exploration of testing and evaluating the robustness of code generation models remains an ongoing endeavor. Previous studies have primarily focused on code generation models specifically for the Python language, overlooking other widely used programming languages. In this work, we conduct a comprehensive comparative analysis to assess the robustness performance of several prominent code generation models and investigate whether robustness can be improved by repairing perturbed docstrings using an LLM. Furthermore, we investigate how their performance varies across different programming languages. To accomplish this, we introduce perturbations in four key areas of the prompt: DocString, function name, syntax, and format. We have compiled and released a dedicated dataset for this purpose. Our results show that all models consistently degrade under perturbations across all three languages, but vary in magnitude depending on the language and perturbation type. Larger model size does not reliably improve robustness, and semantic perturbations prove at least as disruptive as syntactic ones. Our LLM-based docString repair yields only marginal gains for simple perturbations and can degrade performance for semantic ones, highlighting the limits of prompt-level mitigation.

==> declarations.tex <==
\newpage
\section{Declarations}
\subsection{Funding}
\noindent This research was supported by the Fonds de recherche du Québec (Grant No.2024-NOVA346499)\citep{nova}, Natural Sciences and Engineering Research Council of Canada (NSERC) through the Alliance, Grant (Grant No.586838-23), the NSERC Discovery Grant (Grant No. RGPIN-2019-07007 and Grant No. DGECR-2019-00464), and NSERC CREATE Grant (Grant No.555406-2021). We gratefully acknowledge the support of all funding agencies.
\subsection{Ethical approval}
\noindent Not applicable.
\subsection{Informed consent}
\noindent Not applicable.
\subsection{Author Contributions}
\noindent Fazle Rabbi: Conceptualization, Methodology, Experiment, and Writing.\\
Zishuo Ding: Methodology, Writing, and Review.\\
Jinqiu Yang: Supervision, Writing, Review, and Editing. 
\subsection{Data Availability Statement}
\noindent The data used in this study are available in this replication package \footnote{https://github.com/frabbisw/robustextended}.
\subsection{Conflict of Interest}
\noindent Not applicable.
\subsection{Clinical Trial Number}
\noindent Clinical trial number: not applicable.
\newpage
% 8 Declarations
% 8.1 Funding
% Not applicable.
% 8.2 Ethical approval
% Not applicable.
% 8.3 Informed consent
% Not applicable.
% 8.4 Author Contributions
% Fazle Rabbi: Conceptualization, Methodology, Experiment, and Writing.
% Zishuo Ding: Methodology, Writing, and Review.
% Jinqiu Yang: Supervision, Writing, Review, and Editing.
% 8.5 Data Availability Statement
% The data used in this study are available in this replication package6.
% 8.6 Conflict of Interest
% Not applicable.
% 8.7 Clinical Trial Number
% Clinical trial number: not applicable.
